Study of the strong interaction among hadrons with correlations at the LHC

The strong interaction among hadrons has been measured in the past by scattering experiments. Although this technique has been extremely successful in providing information about the nucleon-nucleon and pion-nucleon interactions, when unstable hadrons are considered the experiments become more challenging. In the last few years, the analysis of correlations in the momentum space for pairs of stable and unstable hadrons measured in pp and p-Pb collisions by the ALICE Collaboration at the LHC has provided a new method to investigate the strong interaction among hadrons. In this article, we review the numerous results recently achieved for hyperon-nucleon, hyperon-hyperon, and kaon-nucleon pairs, which show that this new method opens the possibility of measuring the residual strong interaction of any hadron pair.

==> 0_JournalTemplate.tex <==

% Heading 1
\section{INTRODUCTION}
Please begin the main text of your article here. 



%Heading 1
\section{FIRST-LEVEL HEADING}
This is dummy text. 
% Heading 2
\subsection{Second-Level Heading}
This is dummy text. This is dummy text. This is dummy text. This is dummy text.

% Heading 3
\subsubsection{Third-Level Heading}
This is dummy text. This is dummy text. This is dummy text. This is dummy text. 

% Heading 4
\paragraph{Fourth-Level Heading} Fourth-level headings are placed as part of the paragraph.

%Example of a Figure
\section{ELEMENTS\ OF\ THE\ MANUSCRIPT} 
\subsection{Figures}Figures should be cited in the main text in chronological order. This is dummy text with a citation to the first figure (\textbf{Figure \ref{fig1}}). Citations to \textbf{Figure \ref{fig1}} (and other figures) will be bold. 

\begin{figure}[h]
\includegraphics[width=3in]{SampleFigure}
\caption{Figure caption with descriptions of parts a and b}
\label{fig1}
\end{figure}

% Example of a Table
\subsection{Tables} Tables should also be cited in the main text in chronological order (\textbf {Table \ref{tab1}}).

\begin{table}[h]
\tabcolsep7.5pt
\caption{Table caption}
\label{tab1}
\begin{center}
\begin{tabular}{@{}l|c|c|c|c@{}}
\hline
Head 1 &&&&Head 5\\
{(}units)$^{\rm a}$ &Head 2 &Head 3 &Head 4 &{(}units)\\
\hline
Column 1 &Column 2 &Column3$^{\rm b}$ &Column4 &Column\\
Column 1 &Column 2 &Column3 &Column4 &Column\\
Column 1 &Column 2 &Column3 &Column4 &Column\\
Column 1 &Column 2 &Column3 &Column4 &Column\\
\hline
\end{tabular}
\end{center}
\begin{tabnote}
$^{\rm a}$Table footnote; $^{\rm b}$second table footnote.
\end{tabnote}
\end{table}

% Example of lists
\subsection{Lists and Extracts} Here is an example of a numbered list:
\begin{enumerate}
\item List entry number 1,
\item List entry number 2,
\item List entry number 3,\item List entry number 4, and
\item List entry number 5.
\end{enumerate}

Here is an example of a extract.
\begin{extract}
This is an example text of quote or extract.
This is an example text of quote or extract.
\end{extract}

\subsection{Sidebars and Margin Notes}
% Margin Note
\begin{marginnote}[]
\entry{Term A}{definition}
\entry{Term B}{definition}
\entry{Term C}{defintion}
\end{marginnote}

\begin{textbox}[h]\section{SIDEBARS}
Sidebar text goes here.
\subsection{Sidebar Second-Level Heading}
More text goes here.\subsubsection{Sidebar third-level heading}
Text goes here.\end{textbox}



\subsection{Equations}
% Example of a single-line equation
\begin{equation}
a = b \ {\rm ((Single\ Equation\ Numbered))}
\end{equation}
%Example of multiple-line equation
Equations can also be multiple lines as shown in Equations 2 and 3.
\begin{eqnarray}
c = 0 \ {\rm ((Multiple\  Lines, \ Numbered))}\\
ac = 0 \ {\rm ((Multiple \ Lines, \ Numbered))}
\end{eqnarray}

% Summary Points
\begin{summary}[SUMMARY POINTS]
\begin{enumerate}
\item Summary point 1. These should be full sentences.
\item Summary point 2. These should be full sentences.
\item Summary point 3. These should be full sentences.
\item Summary point 4. These should be full sentences.
\end{enumerate}
\end{summary}

% Future Issues
\begin{issues}[FUTURE ISSUES]
\begin{enumerate}
\item Future issue 1. These should be full sentences.
\item Future issue 2. These should be full sentences.
\item Future issue 3. These should be full sentences.
\item Future issue 4. These should be full sentences.
\end{enumerate}
\end{issues}


==> 0_JournalTemplateReferences.tex <==


% Margin notes within bibliography
\section*{LITERATURE\ CITED}

To download the appropriate bibliography style file, please see \url{https://www.annualreviews.org/page/authors/general-information}. 

\\

\noindent
Please see the Style Guide document for instructions on preparing your Literature Cited.

The citations should be numbered in order of appearance. For example:





\begin{verbatim}
\begin{thebibliography}{96}
\expandafter\ifx\csname
natexlab\endcsname\relax\def\natexlab#1{#1}\fi

\bibitem{Glashow:1961tr}
Glashow SL. \textit{Nucl. Phys.} 22:579 (1961)

\bibitem{Weinberg:1967tq}
Weinberg S. \textit{Phys. Rev. Lett.} 19:1264 (1967)

\bibitem{Salam}
Salam A.  In \textit{Elementary Particle Theory: Relativistic
Groups and Analyticity. Proceedings of the 8th Nobel Symposium},
ed. N~Svartholm, p. 367. Stockholm: Almqvist \& Wiksell (1968)
\bibitem{Fritzsch:1973pi}
Fritzsch H, Gell-Mann M, Leutwyler H. \textit{Phys. Lett.} \textit{B} 47:365
(1973)

\bibitem{Gross:1973id}
Gross DJ, Wilczek F. \textit{Phys. Rev. Lett.} 30:1343 (1973)

\bibitem{Politzer:1973fx}
Politzer HD. \textit{Phys. Rev. Lett.} 30:1346 (1973)

\bibitem{Kronfeld:2010bx}
Kronfeld AS, Quigg C. \textit{Am. J. Phys.} 78:1081 (2010)

\bibitem{Langacker:2010}
Langacker P. \textit{The Standard Model and Beyond. Series in
High Energy Physics, Cosmology, and Gravitation}. Boca Raton:
CRC/Taylor \& Francis (2010)

\bibitem{GT2}
Quigg C. \textit{Gauge Theories of the Strong, Weak, and
Electromagnetic Interactions}. Princeton, NJ: Princeton
Univ. Press. 2nd ed. (2013)

\bibitem{MattS}
Schwartz MD. \textit{Quantum Field Theory and the Standard Model}.
Cambridge, UK: Cambridge Univ. Press (2013)

\bibitem{DynSM}
Donoghue JF, Golowich E, Holstein BR. \textit{Dynamics of the
Standard Model}. Cambridge, UK/New York: Cambridge
Univ. Press. 2nd ed. (2014)
\end{thebibliography}
\end{verbatim}

This coding results in the following formatted bibliography:


\begin{thebibliography}{96}
\expandafter\ifx\csname
natexlab\endcsname\relax\def\natexlab#1{#1}\fi

\bibitem{Glashow:1961tr}
Glashow SL. \textit{Nucl. Phys.} 22:579 (1961)

\bibitem{Weinberg:1967tq}
Weinberg S. \textit{Phys. Rev. Lett.} 19:1264 (1967)

\bibitem{Salam}
Salam A.  In \textit{Elementary Particle Theory: Relativistic
Groups and Analyticity. Proceedings of the 8th Nobel Symposium},
ed. N~Svartholm, p. 367. Stockholm: Almqvist \& Wiksell
 (1968)
\bibitem{Fritzsch:1973pi}
Fritzsch H, Gell-Mann M, Leutwyler H. \textit{Phys. Lett.} \textit{B} 47:365
(1973)

\bibitem{Gross:1973id}
Gross DJ, Wilczek F. \textit{Phys. Rev. Lett.} 30:1343 (1973)

\bibitem{Politzer:1973fx}
Politzer HD. \textit{Phys. Rev. Lett.} 30:1346 (1973)

\bibitem{Kronfeld:2010bx}
Kronfeld AS, Quigg C. \textit{Am. J. Phys.} 78:1081 (2010)

\bibitem{Langacker:2010}
Langacker P. \textit{The Standard Model and Beyond. Series in
High Energy Physics, Cosmology, and Gravitation}. Boca Raton:
CRC/Taylor \& Francis (2010)

\bibitem{GT2}
Quigg C. \textit{Gauge Theories of the Strong, Weak, and
Electromagnetic Interactions}. Princeton, NJ: Princeton
Univ. Press. 2nd ed. (2013)

\bibitem{MattS}
Schwartz MD. \textit{Quantum Field Theory and the Standard Model}.
Cambridge, UK: Cambridge Univ. Press (2013)

\bibitem{DynSM}
Donoghue JF, Golowich E, Holstein BR. \textit{Dynamics of the
Standard Model}. Cambridge, UK/New York: Cambridge
Univ. Press. 2nd ed. (2014)

\end{thebibliography}


==> OLD_BibliographyInBibitem.tex <==

% Margin notes within bibliography
%\section*{LITERATURE\ CITED}
\bibliographystyle{ar-style5.bst} 
\begin{thebibliography}{96}
\expandafter\ifx\csname
natexlab\endcsname\relax\def\natexlab#1{#1}\fi
%Introduction
%\cite{HanburyBrown:1956bqd}
\bibitem{HanburyBrown:1956bqd}
R.~Hanbury Brown and R.~Q.~Twiss,
%``A Test of a new type of stellar interferometer on Sirius,''
Nature \textbf{178} (1956), 1046-1048
doi:10.1038/1781046a0
%534 citations counted in INSPIRE as of 06 Oct 2020

% Lambda Lambda
\bibitem{Morita:2014kza}
K.~Morita, T.~Furumoto and A.~Ohnishi,
%``$\Lambda\Lambda$ interaction from relativistic heavy-ion collisions,''
Phys. Rev. C \textbf{91}, no.2, 024916 (2015)
doi:10.1103/PhysRevC.91.024916
[arXiv:1408.6682 [nucl-th]].
\bibitem{Adamczyk:2014vca}
L.~Adamczyk \textit{et al.} [STAR],
%``$\Lambda\Lambda$ Correlation Function in Au+Au collisions at $\sqrt{s_{NN}}=$ 200 GeV,''
Phys. Rev. Lett. \textbf{114}, no.2, 022301 (2015)
doi:10.1103/PhysRevLett.114.022301
[arXiv:1408.4360 [nucl-ex]].
%\cite{Lednicky:1981su}
\bibitem{Ohnishi:2016elb}
A.~Ohnishi, K.~Morita, K.~Miyahara and T.~Hyodo,
%``Hadron\textendash{}hadron correlation and interaction from heavy\textendash{}ion collisions,''
Nucl. Phys. A \textbf{954}, 294-307 (2016)
doi:10.1016/j.nuclphysa.2016.05.010
[arXiv:1603.05761 [nucl-th]].
\bibitem{Lednicky:1981su}
R.~Lednicky and V.~L.~Lyuboshits,
%``Final State Interaction Effect on Pairing Correlations Between Particles with Small Relative Momenta,''
Sov. J. Nucl. Phys. \textbf{35} (1982), 770
JINR-E2-81-453.
%300 citations counted in INSPIRE as of 23 Sep 2020

\bibitem{Beane:2013br}
{\bfseries NPLQCD} Collaboration, S.~Beane {\em et~al.}, ``{Nucleon-Nucleon
  Scattering Parameters in the Limit of SU(3) Flavor Symmetry}'',
  \href{http://dx.doi.org/10.1103/PhysRevC.88.024003}{{\em Phys. Rev. C}
  {\bfseries 88} no.~2, (2013) 024003},
  \href{http://arxiv.org/abs/1301.5790}{{\ttfamily arXiv:1301.5790 [hep-lat]}}.

\bibitem{Epelbaum:2009pd}
E.~Epelbaum, H.~Krebs, D.~Lee, and U.-G. Meissner, ``{Lattice effective field
  theory calculations for A = 3,4,6,12 nuclei}'',
  \href{http://dx.doi.org/10.1103/PhysRevLett.104.142501}{{\em Phys. Rev. Lett.} {\bfseries 104} (2010) 142501},
  \href{http://arxiv.org/abs/0912.4195}{{\ttfamily arXiv:0912.4195 [nucl-th]}}.

\bibitem{Eisele:1971mk}
F.~Eisele, H.~Filthuth, W.~Foehlisch, V.~Hepp, and G.~Zech, ``{Elastic
  $\Sigma^{\pm}$p scattering at low energies}'',
  \href{http://dx.doi.org/10.1016/0370-2693(71)90053-0}{{\em Phys. Lett. B}
  {\bfseries 37} (1971) 204--206}.

\bibitem{Alexander:1969cx}
G.~Alexander, U.~Karshon, A.~Shapira, G.~Yekutieli, R.~Engelmann, H.~Filthuth,
  and W.~Lughofer, ``{Study of the $\Lambda\mbox{--}N$ system in low-energy
  $\Lambda\mbox{--}p$ elastic scattering}'',
  \href{http://dx.doi.org/10.1103/PhysRev.173.1452}{{\em Phys. Rev.} {\bfseries
  173} (1968) 1452--1460}.

\bibitem{SechiZorn:1969hk}
B.~Sechi-Zorn, B.~Kehoe, J.~Twitty, and R.~Burnstein, ``{Low-energy
  $\Lambda$--proton elastic scattering}'',
  \href{http://dx.doi.org/10.1103/PhysRev.175.1735}{{\em Phys. Rev.} {\bfseries
  175} (1968) 1735--1740}.

\bibitem{Muller:1972cq}
R.~Muller, ``{Observation of cascade hyperon interactions}'',
  \href{http://dx.doi.org/10.1016/0370-2693(72)90757-5}{{\em Phys. Lett. B}
  {\bfseries 38} (1972) 123--124}.

\bibitem{PhysRevC.47.761}
V.~Stoks and J.~de~Swart, ``{Comparison of potential models with the pp
  scattering data below 350 MeV}'',
  \href{http://dx.doi.org/10.1103/PhysRevC.47.761}{{\em Phys. Rev. C}
  {\bfseries 47} (1993) 761--767}.

\bibitem{FemtoRun1}
{\bfseries ALICE} Collaboration, S.~Acharya {\em et~al.}, ``{p-p, p-$\Lambda$
  and $\Lambda$-$\Lambda$ correlations studied via femtoscopy in pp reactions
  at $\sqrt{s}$ = 7 TeV}'',
  \href{http://dx.doi.org/10.1103/PhysRevC.99.024001}{{\em Phys. Rev. C}
  {\bfseries 99} (2019) 024001}.

\bibitem{Acharya:2019bsa}
{\bfseries ALICE} Collaboration, S.~Acharya {\em et~al.}, ``{Scattering studies
  with low-energy kaon-proton femtoscopy in proton-proton collisions at the
  LHC}'', \href{http://dx.doi.org/10.1103/PhysRevLett.124.092301}{{\em Phys.
  Rev. Lett.} {\bfseries 124} (2020) 092301}.

\bibitem{FemtoLambdaLambda}
{\bfseries ALICE} Collaboration, S.~Acharya {\em et~al.}, ``{Study of the
  $\Lambda$--$\Lambda$ interaction with femtoscopy correlations in pp and p--Pb
  collisions at the LHC}'',
  \href{http://dx.doi.org/10.1016/j.physletb.2019.134822}{{\em Phys. Lett.}
  {\bfseries B797} (2019) 134822}.

\bibitem{FemtopXi}
{\bfseries ALICE} Collaboration, S.~Acharya {\em et~al.}, ``{First Observation
  of an Attractive Interaction between a Proton and a Cascade Baryon}'',
  \href{http://dx.doi.org/10.1103/PhysRevLett.123.112002}{{\em Phys. Rev.
  Lett.} {\bfseries 123} (2019) 112002}.

\bibitem{Acharya:2019kqn}
{\bfseries ALICE} Collaboration, S.~Acharya {\em et~al.}, ``{Investigation of
  the p-$\Sigma^{0}$ interaction via femtoscopy in pp collisions}'',
  \href{http://dx.doi.org/10.1016/j.physletb.2020.135419}{{\em Phys. Lett. B}{\bfseries 805} (2020) 135419}.

\bibitem{Iritani:2018sra}
{\bfseries HAL QCD} Collaboration, T.~Iritani {\em et~al.}, ``{$N\Omega$
  dibaryon from lattice QCD near the physical point}'',
  \href{http://dx.doi.org/10.1016/j.physletb.2019.03.050}{{\em Phys. Lett. B}
  {\bfseries 792} (2019) 284--289}.

\bibitem{Sasaki:2019qnh}
K.~Sasaki {\em et~al.}, ``{$\Lambda\Lambda$ and N$\Xi$ interactions from
  Lattice QCD near the physical point}'',
  \href{http://dx.doi.org/10.1016/j.nuclphysa.2020.121737}{{\em Nucl. Phys. A}
  {\bfseries 998} (2020) 121737}.

\bibitem{Acharya:2020dfb}
{\bfseries ALICE} Collaboration, S.~Acharya {\em et~al.}, ``{Search for a
  common baryon source in high-multiplicity pp collisions at the LHC}'',
  \href{http://arxiv.org/abs/2004.08018}{{\ttfamily arXiv:2004.08018
  [nucl-ex]}}. {Submitted to $Phys. Lett. B$}.

\bibitem{RevModPhys.81.1773}
E.~Epelbaum, H.-W. Hammer, and U.-G. Meissner, ``{Modern Theory of Nuclear
  Forces}'', \href{http://dx.doi.org/10.1103/RevModPhys.81.1773}{{\em Rev. Mod.
  Phys.} {\bfseries 81} (2009) 1773--1825}.

\bibitem{Hebeler:2015hla}
K.~Hebeler, J.~Holt, J.~Menendez, and A.~Schwenk, ``{Nuclear forces and their
  impact on neutron-rich nuclei and neutron-rich matter}'',
  \href{http://dx.doi.org/10.1146/annurev-nucl-102313-025446}{{\em Ann. Rev.
  Nucl. Part. Sci.} {\bfseries 65} (2015) 457--484}.

\bibitem{PhysRevLett.118.152503}
E.~Gebrerufael, K.~Vobig, H.~Hergert, and R.~Roth, ``{Ab Initio Description of
  Open-Shell Nuclei: Merging No-Core Shell Model and In-Medium Similarity
  Renormalization Group}'',
  \href{http://dx.doi.org/10.1103/PhysRevLett.118.152503}{{\em Phys. Rev.
  Lett.} {\bfseries 118} (2017) 152503}.

\bibitem{Klijnsma:2017eqp}
T.~Klijnsma, S.~Bethke, G.~Dissertori, and G.~P. Salam, ``{Determination of the
  strong coupling constant $\alpha_s(m_Z)$ from measurements of the total cross
  section for top-antitop quark production}'',
  \href{http://dx.doi.org/10.1140/epjc/s10052-017-5340-5}{{\em Eur. Phys. J. C}
  {\bfseries 77} (2017) 778}.

\bibitem{Orginos:2015aya}
K.~Orginos, A.~Parreno, M.~J. Savage, S.~R. Beane, E.~Chang, and W.~Detmold,
  ``{Two nucleon systems at $m_\pi\sim 450~{\rm MeV}$ from lattice QCD}'',
  \href{http://dx.doi.org/10.1103/PhysRevD.92.114512}{{\em Phys. Rev. D}
  {\bfseries 92} (2015) 114512}.

\bibitem{Wagman:2017tmp}
M.~L. Wagman, F.~Winter, E.~Chang, Z.~Davoudi, W.~Detmold, K.~Orginos, M.~J.
  Savage, and P.~E. Shanahan, ``{Baryon-Baryon Interactions and Spin-Flavor
  Symmetry from Lattice Quantum Chromodynamics}'',
  \href{http://dx.doi.org/10.1103/PhysRevD.96.114510}{{\em Phys. Rev. D}
  {\bfseries 96} no.~11, (2017) 114510},
  \href{http://arxiv.org/abs/1706.06550}{{\ttfamily arXiv:1706.06550
  [hep-lat]}}.

\bibitem{Hatsuda:2018nes}
T.~Hatsuda, ``{Lattice quantum chromodynamics and baryon-baryon
  interactions}'', \href{http://dx.doi.org/10.1007/s11467-018-0829-4}{{\em
  Front. Phys. (Beijing)} {\bfseries 13} (2018) 132105}.

\bibitem{Hashimoto:2006aw}
O.~Hashimoto and H.~Tamura, ``{Spectroscopy of $\Lambda$ hypernuclei}'',
  \href{http://dx.doi.org/10.1016/j.ppnp.2005.07.001}{{\em Prog. Part. Nucl.
  Phys.} {\bfseries 57} (2006) 564--653}.

\bibitem{Nakazawa:2015joa}
K.~Nakazawa {\em et~al.}, ``{The first evidence of a deeply bound state of
  Xi$^{-}$--$^{14}$N system}'',
  \href{http://dx.doi.org/10.1093/ptep/ptv008}{{\em PTEP} {\bfseries 2015}
  (2015) 033D02}.

\bibitem{Nagae:2017slp}
T.~Nagae {\em et~al.}, ``{Search For A $\Xi$ Bound State In The
  $^{12}$C($K^-$,$K^+$)$X$ Reaction At 1.8 GeV/c in J-PARC}'',
  \href{http://dx.doi.org/10.22323/1.281.0038}{{\em PoS} {\bfseries INPC2016}
  (2017) 038}.

\bibitem{Francis:2018qch}
A.~Francis, J.~Green, P.~Junnarkar, C.~Miao, T.~Rae, and H.~Wittig, ``{Lattice
  QCD study of the $H$ dibaryon using hexaquark and two-baryon
  interpolators}'', \href{http://dx.doi.org/10.1103/PhysRevD.99.074505}{{\em
  Phys. Rev. D} {\bfseries 99} no.~7, (2019) 074505},
  \href{http://arxiv.org/abs/1805.03966}{{\ttfamily arXiv:1805.03966
  [hep-lat]}}.
%\cite{Takahashi:2001nm}
\bibitem{Jaffe:1976yi}
R.~L. Jaffe, ``{Perhaps a Stable Dihyperon}'',
  \href{http://dx.doi.org/10.1103/PhysRevLett.38.195}{{\em Phys. Rev. Lett.}
  {\bfseries 38} (1977) 195--198}. [Erratum: Phys.Rev.Lett. 38, 617 (1977)].
\bibitem{Takahashi:2001nm}
  H.~Takahashi {\it et al.},
  %``Observation of a (Lambda Lambda)He-6 double hypernucleus,''
  Phys.\ Rev.\ Lett.\  {\bf 87} (2001) 212502.
  doi:10.1103/PhysRevLett.87.212502
  %%CITATION = doi:10.1103/PhysRevLett.87.212502;%%
  %437 citations counted in INSPIRE as of 01 Oct 2020
\bibitem{PhysRevD.15.2547}
M.~M. Nagels, T.~A. Rijken, and J.~J. de~Swart, ``{Baryon-baryon scattering in
  a one-boson-exchange-potential approach. II. Hyperon-nucleon scattering}'',
  \href{http://dx.doi.org/10.1103/PhysRevD.15.2547}{{\em Phys. Rev. D}
  {\bfseries 15} (1977) 2547--2564}.

\bibitem{PhysRevD.20.1633}
M.~M. Nagels, T.~A. Rijken, and J.~J. de~Swart, ``{Baryon-baryon scattering in
  a one-boson-exchange-potential approach. III. A nucleon-nucleon and
  hyperon-nucleon analysis including contributions of a nonet of scalar
  mesons}'', \href{http://dx.doi.org/10.1103/PhysRevD.20.1633}{{\em Phys. Rev.
  D} {\bfseries 20} (1979) 1633--1645}.

\bibitem{Gongyo:2017fjb}
S.~Gongyo {\em et~al.}, ``{Most Strange Dibaryon from Lattice QCD}'',
  \href{http://dx.doi.org/10.1103/PhysRevLett.120.212001}{{\em Phys. Rev.
  Lett.} {\bfseries 120} no.~21, (2018) 212001},
  \href{http://arxiv.org/abs/1709.00654}{{\ttfamily arXiv:1709.00654
  [hep-lat]}}.

\bibitem{Adam:2015nca}
{\bfseries ALICE} Collaboration, J.~Adam {\em et~al.}, ``{Search for weakly
  decaying $\overline{\Lambda\mathrm{n}}$ and $\Lambda\Lambda $ exotic bound
  states in central Pb-Pb collisions at $\sqrt{s_{\textrm{NN}}}$ = 2.76 TeV}'',
  \href{http://dx.doi.org/10.1016/j.physletb.2015.11.048}{{\em Phys. Lett. B}
  {\bfseries 752} (2016) 267--277}.

\bibitem{Kim:2013vym}
{\bfseries Belle} Collaboration, B.~Kim {\em et~al.}, ``{Search for an
  $H$-dibaryon with mass near $2m_\Lambda$ in $\Upsilon(1S)$ and $\Upsilon(2S)$
  decays}'', \href{http://dx.doi.org/10.1103/PhysRevLett.110.222002}{{\em Phys.
  Rev. Lett.} {\bfseries 110} (2013) 222002}.

\bibitem{Chrien:1998yt}
R.~Chrien, ``{H particle searches at Brookhaven}'',
  \href{http://dx.doi.org/10.1016/S0375-9474(97)00714-8}{{\em Nucl. Phys. A}
  {\bfseries 629} (1998) 388C--397C}.

\bibitem{Yoon:2007aq}
C.~Yoon {\em et~al.}, ``{Search for the H-dibaryon resonance in $^{12}$C
  ($K^{-}$, $K^{+}\Lambda\,\Lambda\,X$)}'',
  \href{http://dx.doi.org/10.1103/PhysRevC.75.022201}{{\em Phys. Rev. C}
  {\bfseries 75} (2007) 022201}.

\bibitem{Ahn:1998fj}
{\bfseries KEK-PS E224} Collaboration, J.~Ahn {\em et~al.}, ``{Enhanced
  $\Lambda\,\Lambda$ production near threshold in the $^{12}$C($K^{-},K^{+}$)
  reaction}'', \href{http://dx.doi.org/10.1016/S0370-2693(98)01416-6}{{\em
  Phys. Lett. B} {\bfseries 444} (1998) 267--272}.

\bibitem{Tolos:2020aln}
L.~Tolos and L.~Fabbietti, ``{Strangeness in Nuclei and Neutron Stars}'',
  \href{http://dx.doi.org/10.1016/j.ppnp.2020.103770}{{\em Prog. Part. Nucl.
  Phys.} {\bfseries 112} (2020) 103770},
  \href{http://arxiv.org/abs/2002.09223}{{\ttfamily arXiv:2002.09223
  [nucl-ex]}}.

\bibitem{Adamczewski-Musch:2016jlh}
{\bfseries HADES} Collaboration, J.~Adamczewski-Musch {\em et~al.}, ``{The
  $\bf{\Lambda p}$ interaction studied via femtoscopy in p + Nb reactions at
  $\mathbf{\sqrt{s_{NN}}=3.18} ~\mathrm{\bf{GeV}}$}'',
  \href{http://dx.doi.org/10.1103/PhysRevC.94.025201}{{\em Phys. Rev. C}
  {\bfseries 94} no.~2, (2016) 025201},
  \href{http://arxiv.org/abs/1602.08880}{{\ttfamily arXiv:1602.08880
  [nucl-ex]}}.

\bibitem{ALICE:2017jyt}
{\bfseries ALICE} Collaboration, J.~Adam {\em et~al.}, ``{Enhanced production
  of multi-strange hadrons in high-multiplicity proton-proton collisions}'',
  \href{http://dx.doi.org/10.1038/nphys4111}{{\em Nature Phys.} {\bfseries 13}
  (2017) 535--539}.

\bibitem{Mihaylov:2018rva}
D.~Mihaylov, V.~Mantovani~Sarti, O.~Arnold, L.~Fabbietti, B.~Hohlweger, and
  A.~Mathis, ``{A femtoscopic Correlation Analysis Tool using the Schr\"odinger
  equation (CATS)}'',
  \href{http://dx.doi.org/10.1140/epjc/s10052-018-5859-0}{{\em Eur. Phys. J. C}
  {\bfseries 78} (2018) 394}.

\bibitem{Adamczyk:2014vca}
{\bfseries STAR} Collaboration, L.~Adamczyk {\em et~al.}, ``{$\Lambda\Lambda$
  Correlation Function in Au+Au collisions at $\sqrt{s_{\textrm{NN}}}=$ 200
  GeV}'', \href{http://dx.doi.org/10.1103/PhysRevLett.114.022301}{{\em Phys.
  Rev. Lett.} {\bfseries 114} (2015) 022301}.

\bibitem{Morita:2014kza}
K.~Morita, T.~Furumoto, and A.~Ohnishi, ``{$\Lambda\Lambda$ interaction from
  relativistic heavy-ion collisions}'',
  \href{http://dx.doi.org/10.1103/PhysRevC.91.024916}{{\em Phys. Rev. C}
  {\bfseries 91} (2015) 024916}.

\bibitem{STAR:2018uho}
{\bfseries STAR} Collaboration, J.~Adam {\em et~al.}, ``{The Proton-$\Omega$
  correlation function in Au\,+\,Au collisions at
  $\sqrt{s_{\textrm{NN}}}$\,=\,200 GeV}'',
  \href{http://dx.doi.org/10.1016/j.physletb.2019.01.055}{{\em Phys. Lett. B}
  {\bfseries 790} (2019) 490--497}.

\bibitem{Pratt:1986cc}
S.~Pratt, ``{Pion Interferometry of Quark-Gluon Plasma}'',
  \href{http://dx.doi.org/10.1103/PhysRevD.33.1314}{{\em Phys. Rev. D}
  {\bfseries 33} (1986) 1314--1327}.

\bibitem{Lisa:2005dd}
M.~A. Lisa, S.~Pratt, R.~Soltz, and U.~Wiedemann, ``{Femtoscopy in relativistic
  heavy ion collisions}'',
  \href{http://dx.doi.org/10.1146/annurev.nucl.55.090704.151533}{{\em Ann. Rev.
  Nucl. Part. Sci.} {\bfseries 55} (2005) 357--402}.

\bibitem{Haidenbauer:2019utu}
J.~Haidenbauer and U.-G. Meißner, ``{Phenomenological view on baryon-baryon
  potentials from lattice QCD simulations}'',
  \href{http://dx.doi.org/10.1140/epja/i2019-12736-0}{{\em Eur. Phys. J. A}
  {\bfseries 55} no.~5, (2019) 70},
  \href{http://arxiv.org/abs/1901.01801}{{\ttfamily arXiv:1901.01801
  [nucl-th]}}.

\bibitem{Morita:2016auo}
K.~Morita, A.~Ohnishi, F.~Etminan, and T.~Hatsuda, ``{Probing multistrange
  dibaryons with proton-omega correlations in high-energy heavy ion
  collisions}'', \href{http://dx.doi.org/10.1103/PhysRevC.94.031901}{{\em Phys.
  Rev. C} {\bfseries 94} no.~3, (2016) 031901},
  \href{http://arxiv.org/abs/1605.06765}{{\ttfamily arXiv:1605.06765
  [hep-ph]}}. [Erratum: Phys.Rev.C 100, 069902 (2019)].

\bibitem{Morita:2019rph}
K.~Morita, S.~Gongyo, T.~Hatsuda, T.~Hyodo, Y.~Kamiya, and A.~Ohnishi,
  ``{Probing $\Omega\Omega$ and $p\Omega$ dibaryons with femtoscopic
  correlations in relativistic heavy-ion collisions}'',
  \href{http://dx.doi.org/10.1103/PhysRevC.101.015201}{{\em Phys. Rev. C}
  {\bfseries 101} (2020) 015201}.

\bibitem{Abelevetal:2014cna}
{\bfseries ALICE} Collaboration, B.~Abelev {\em et~al.}, ``{Upgrade of the
  ALICE Experiment: Letter Of Intent}'',
  \href{http://dx.doi.org/10.1088/0954-3899/41/8/087001}{{\em J. Phys. G}
  {\bfseries 41} (2014) 087001}.

\bibitem{YellowReport_better}
Z.~Citron {\em et~al.}, ``{Report from Working Group 5}: {Future physics
  opportunities for high-density QCD at the LHC with heavy-ion and proton
  beams}'', \href{http://dx.doi.org/10.23731/CYRM-2019-007.1159}{{\em CERN
  Yellow Rep. Monogr.} {\bfseries 7} (2019) 1159--1410}.

\bibitem{Aamodt:2008zz}
{\bfseries ALICE} Collaboration, K.~Aamodt {\em et~al.}, ``{The ALICE
  experiment at the CERN LHC}'',
  \href{http://dx.doi.org/10.1088/1748-0221/3/08/S08002}{{\em JINST} {\bfseries
  3} (2008) S08002}.

\bibitem{Abelev:2014ffa}
{\bfseries ALICE} Collaboration, B.~Abelev {\em et~al.}, ``{Performance of the
  ALICE Experiment at the CERN LHC}'',
  \href{http://dx.doi.org/10.1142/S0217751X14300440}{{\em Int. J. Mod. Phys.}
  {\bfseries A29} (2014) 1430044}.

\bibitem{Abbas:2013taa}
{\bfseries ALICE} Collaboration, E.~Abbas {\em et~al.}, ``{Performance of the
  ALICE VZERO system}'',
  \href{http://dx.doi.org/10.1088/1748-0221/8/10/P10016}{{\em JINST} {\bfseries
  8} (2013) P10016}.

\bibitem{Acharya:2019kyh}
{\bfseries ALICE} Collaboration, S.~Acharya {\em et~al.}, ``{Multiplicity
  dependence of (multi-)strange hadron production in proton-proton collisions
  at $\sqrt{s}$ = 13 TeV}'',
  \href{http://dx.doi.org/10.1140/epjc/s10052-020-7673-8}{{\em Eur. Phys. J. C}
  {\bfseries 80} (2020) 167}.

\bibitem{Aamodt:2010aa}
{\bfseries ALICE} Collaboration, K.~Aamodt {\em et~al.}, ``{Alignment of the
  ALICE Inner Tracking System with cosmic-ray tracks}'',
  \href{http://dx.doi.org/10.1088/1748-0221/5/03/P03003}{{\em JINST} {\bfseries
  5} (2010) P03003}.

\bibitem{Alme:2010ke}
J.~Alme {\em et~al.}, ``{The ALICE TPC, a large 3-dimensional tracking device
  with fast readout for ultra-high multiplicity events}'',
  \href{http://dx.doi.org/10.1016/j.nima.2010.04.042}{{\em Nucl. Instrum. Meth.
  A} {\bfseries 622} (2010) 316--367}.

\bibitem{Akindinov:2013tea}
A.~Akindinov {\em et~al.}, ``{Performance of the ALICE Time-Of-Flight detector
  at the LHC}'', \href{http://dx.doi.org/10.1140/epjp/i2013-13044-x}{{\em Eur.
  Phys. J. Plus} {\bfseries 128} (2013) 44}.

\bibitem{Tanabashi:2018oca}
{\bfseries Particle Data Group} Collaboration, M.~Tanabashi {\em et~al.},
  ``{Review of Particle Physics}'',
\href{http://dx.doi.org/10.1103/PhysRevD.98.030001}{{\em Phys. Rev.} {\bfseries
  D98} (2018) 030001}.
%%CITATION = PHRVA,D98,030001;%%.

\bibitem{Aamodt:2011zza}
{\bfseries ALICE} Collaboration, K.~Aamodt {\em et~al.}, ``{Strange particle
  production in proton-proton collisions at sqrt(s) = 0.9 TeV with ALICE at the
  LHC}'', \href{http://dx.doi.org/10.1140/epjc/s10052-011-1594-5}{{\em Eur.
  Phys. J. C} {\bfseries 71} (2011) 1594}.

\bibitem{PhysRevC.89.054916}
A.~Kisiel, H.~Zbroszczyk, and M.~Szyma\ifmmode~\acute{n}\else \'{n}\fi{}ski,
  ``Extracting baryon-antibaryon strong-interaction potentials from
  $p\overline{\ensuremath{\Lambda}}$ femtoscopic correlation functions'',
  \href{http://dx.doi.org/10.1103/PhysRevC.89.054916}{{\em Phys. Rev. C}
  {\bfseries 89} (2014) 054916}.

%\cite{Acharya:2017qtq}
\bibitem{Acharya:2017qtq}
S.~Acharya \textit{et al.} [ALICE],
%``Kaon femtoscopy in Pb-Pb collisions at $\sqrt{s_{\rm{NN}}}$ = 2.76 TeV,''
Phys. Rev. C \textbf{96} (2017) no.6, 064613
doi:10.1103/PhysRevC.96.064613
[arXiv:1709.01731 [nucl-ex]].
%16 citations counted in INSPIRE as of 23 Sep 2020

%source Chapter
%\cite{Bearden:2000ex}
\bibitem{Bearden:2000ex}
I.~G.~Bearden and others,
%``Space-time evolution of the hadronic source in peripheral to central Pb + Pb collisions,''
Eur. Phys. J. C \textbf{18} (2000), 317-325
doi:10.1007/s100520000543
%12 citations counted in INSPIRE as of 23 Sep 2020

%\cite{Wiedemann:1996ig}
\bibitem{WiedemannHeinz}
U.~A.~Wiedemann and U.~W.~Heinz,
%``Resonance contributions to HBT correlation radii,''
Phys. Rev. C \textbf{56} (1997), 3265-3286
doi:10.1103/PhysRevC.56.3265
[arXiv:nucl-th/9611031 [nucl-th]].
%115 citations counted in INSPIRE as of 23 Sep 2020

%\cite{Wiringa:1994wb}
\bibitem{Wiringa:1994wb}
R.~B.~Wiringa, V.~G.~J.~Stoks and R.~Schiavilla,
%``An Accurate nucleon-nucleon potential with charge independence breaking,''
Phys. Rev. C \textbf{51} (1995), 38-51
doi:10.1103/PhysRevC.51.38
[arXiv:nucl-th/9408016 [nucl-th]].
%2617 citations counted in INSPIRE as of 25 Sep 2020

%\cite{Polinder:2006zh}
\bibitem{POLINDER2006244}
H.~Polinder, J.~Haidenbauer and U.~G.~Meissner,
%``Hyperon-nucleon interactions: A Chiral effective field theory approach,''
Nucl. Phys. A \textbf{779} (2006), 244-266
doi:10.1016/j.nuclphysa.2006.09.006
[arXiv:nucl-th/0605050 [nucl-th]].
%177 citations counted in INSPIRE as of 25 Sep 2020

%\cite{Haidenbauer:2019boi}
\bibitem{Haidenbauer:2019boi}
J.~Haidenbauer, U.~G.~Mei\ss{}ner and A.~Nogga,
%``Hyperon\textendash{}nucleon interaction within chiral effective field theory revisited,''
Eur. Phys. J. A \textbf{56} (2020) no.3, 91
doi:10.1140/epja/s10050-020-00100-4
[arXiv:1906.11681 [nucl-th]].
%23 citations counted in INSPIRE as of 25 Sep 2020

%\cite{Adam:2015vja}
\bibitem{Adam:2015vja}
J.~Adam \textit{et al.} [ALICE],
%``One-dimensional pion, kaon, and proton femtoscopy in Pb-Pb collisions at $\sqrt{s_{\rm {NN}}}$ =2.76 TeV,''
Phys. Rev. C \textbf{92} (2015) no.5, 054908
doi:10.1103/PhysRevC.92.054908
[arXiv:1506.07884 [nucl-ex]].
%46 citations counted in INSPIRE as of 25 Sep 2020

%K-K and π-π pp
%\cite{Sirunyan:2017ies}
\bibitem{Sirunyan:2017ies}
A.~M.~Sirunyan \textit{et al.} [CMS],
%``Bose-Einstein correlations in $pp, p\mathrm{Pb}$, and PbPb collisions at $\sqrt{{s}_{NN}}=0.9-7$ TeV,''
Phys. Rev. C \textbf{97} (2018) no.6, 064912
doi:10.1103/PhysRevC.97.064912
[arXiv:1712.07198 [hep-ex]].
%23 citations counted in INSPIRE as of 25 Sep 2020

%\cite{Aad:2015sja}
\bibitem{Aad:2015sja}
G.~Aad \textit{et al.} [ATLAS],
%``Two-particle Bose\textendash{}Einstein correlations in pp collisions at $\mathbf {\sqrt{s} =}$ 0.9 and 7 TeV measured with the ATLAS detector,''
Eur. Phys. J. C \textbf{75} (2015) no.10, 466
doi:10.1140/epjc/s10052-015-3644-x
[arXiv:1502.07947 [hep-ex]].
%58 citations counted in INSPIRE as of 25 Sep 2020

%\cite{Abelev:2012sq}
\bibitem{Abelev:2012sq}
B.~Abelev \textit{et al.} [ALICE],
%``Charged kaon femtoscopic correlations in $pp$ collisions at $\sqrt{s}=7$ TeV,''
Phys. Rev. D \textbf{87} (2013) no.5, 052016
doi:10.1103/PhysRevD.87.052016
[arXiv:1212.5958 [hep-ex]].
%28 citations counted in INSPIRE as of 25 Sep 2020

%\cite{Abelev:2012ms}
\bibitem{Abelev:2012ms}
B.~Abelev \textit{et al.} [ALICE],
%``$K^0_s-K^0_s$ correlations in $pp$ collisions at $\sqrt{s}=7$ TeV from the LHC ALICE experiment,''
Phys. Lett. B \textbf{717} (2012), 151-161
doi:10.1016/j.physletb.2012.09.013
[arXiv:1206.2056 [hep-ex]].
%25 citations counted in INSPIRE as of 25 Sep 2020

%\cite{Sirunyan:2019umv}
\bibitem{Sirunyan:2019umv}
A.~M.~Sirunyan \textit{et al.} [CMS],
%``Bose-Einstein correlations of charged hadrons in proton-proton collisions at $\sqrt{s} =$ 13 TeV,''
JHEP \textbf{03} (2020), 014
doi:10.1007/JHEP03(2020)014
[arXiv:1910.08815 [hep-ex]].
%4 citations counted in INSPIRE as of 25 Sep 2020

%\cite{Khachatryan:2016txc}
\bibitem{Khachatryan:2016txc}
V.~Khachatryan \textit{et al.} [CMS],
%``Evidence for collectivity in pp collisions at the LHC,''
Phys. Lett. B \textbf{765} (2017), 193-220
doi:10.1016/j.physletb.2016.12.009
[arXiv:1606.06198 [nucl-ex]].
%261 citations counted in INSPIRE as of 25 Sep 2020

%\cite{Khachatryan:2010gv}
\bibitem{Khachatryan:2010gv}
V.~Khachatryan \textit{et al.} [CMS],
%``Observation of Long-Range Near-Side Angular Correlations in Proton-Proton Collisions at the LHC,''
JHEP \textbf{09} (2010), 091
doi:10.1007/JHEP09(2010)091
[arXiv:1009.4122 [hep-ex]].
%881 citations counted in INSPIRE as of 25 Sep 2020

%\cite{ALICE:2017jyt}
\bibitem{Livio}
J.~Adam \textit{et al.} [ALICE],
%``Enhanced production of multi-strange hadrons in high-multiplicity proton-proton collisions,''
Nature Phys. \textbf{13} (2017), 535-539
doi:10.1038/nphys4111
[arXiv:1606.07424 [nucl-ex]].
%331 citations counted in INSPIRE as of 25 Sep 2020

%\cite{Acharya:2018orn}
\bibitem{Acharya:2018orn}
S.~Acharya \textit{et al.} [ALICE],
%``Multiplicity dependence of light-flavor hadron production in pp collisions at $\sqrt{s}$ = 7 TeV,''
Phys. Rev. C \textbf{99} (2019) no.2, 024906
doi:10.1103/PhysRevC.99.024906
[arXiv:1807.11321 [nucl-ex]].
%67 citations counted in INSPIRE as of 25 Sep 2020

%\cite{TFist}
\bibitem{TFist}
V.~Vovchenko and H.~Stoecker,
%``Thermal-FIST: A package for heavy-ion collisions and hadronic equation of state,''
Comput. Phys. Commun. \textbf{244} (2019), 295-310
doi:10.1016/j.cpc.2019.06.024
[arXiv:1901.05249 [nucl-th]].
%20 citations counted in INSPIRE as of 25 Sep 2020

%\cite{Becattini:2001fg}
\bibitem{Becattini:2001fg}
F.~Becattini and G.~Passaleva,
%``Statistical hadronization model and transverse momentum spectra of hadrons in high-energy collisions,''
Eur. Phys. J. C \textbf{23} (2002), 551-583
doi:10.1007/s100520100869
[arXiv:hep-ph/0110312 [hep-ph]].
%115 citations counted in INSPIRE as of 25 Sep 2020

%\cite{Wheaton:2004qb}
\bibitem{Wheaton:2004qb}
S.~Wheaton and J.~Cleymans,
%``THERMUS: A Thermal model package for ROOT,''
Comput. Phys. Commun. \textbf{180} (2009), 84-106
doi:10.1016/j.cpc.2008.08.001
[arXiv:hep-ph/0407174 [hep-ph]].
%322 citations counted in INSPIRE as of 25 Sep 2020

%\cite{Pierog:2013ria}
\bibitem{Pierog:2013ria}
T.~Pierog, I.~Karpenko, J.~M.~Katzy, E.~Yatsenko and K.~Werner,
%``EPOS LHC: Test of collective hadronization with data measured at the CERN Large Hadron Collider,''
Phys. Rev. C \textbf{92} (2015) no.3, 034906
doi:10.1103/PhysRevC.92.034906
[arXiv:1306.0121 [hep-ph]].
%780 citations counted in INSPIRE as of 25 Sep 2020


%Coupled-channel dynamics
%\cite{Haidenbauer:2018jvl}
\bibitem{Haidenbauer:2018jvl}
J.~Haidenbauer,
%``Coupled-channel effects in hadron\textendash{}hadron correlation functions,''
Nucl. Phys. A \textbf{981} (2019), 1-16
doi:10.1016/j.nuclphysa.2018.10.090
[arXiv:1808.05049 [hep-ph]].
%11 citations counted in INSPIRE as of 25 Sep 2020

%\cite{Kamiya:2019uiw}
\bibitem{Kamiya:2019uiw}
Y.~Kamiya, T.~Hyodo, K.~Morita, A.~Ohnishi and W.~Weise,
%``$K^-p$ Correlation Function from High-Energy Nuclear Collisions and Chiral SU(3) Dynamics,''
Phys. Rev. Lett. \textbf{124} (2020) no.13, 132501
doi:10.1103/PhysRevLett.124.132501
[arXiv:1911.01041 [nucl-th]].
%2 citations counted in INSPIRE as of 25 Sep 2020

%\cite{Lednicky:1981su}
\bibitem{Lednicky:1981su}
R.~Lednicky and V.~L.~Lyuboshits,
%``Final State Interaction Effect on Pairing Correlations Between Particles with Small Relative Momenta,''
Sov. J. Nucl. Phys. \textbf{35} (1982), 770
JINR-E2-81-453.
%300 citations counted in INSPIRE as of 28 Sep 2020

%\cite{Hall:2014uca}
\bibitem{Lambda1405_lat}
J.~M.~M.~Hall, W.~Kamleh, D.~B.~Leinweber, B.~J.~Menadue, B.~J.~Owen, A.~W.~Thomas and R.~D.~Young,
%``Lattice QCD Evidence that the \ensuremath{\Lambda}(1405) Resonance is an Antikaon-Nucleon Molecule,''
Phys. Rev. Lett. \textbf{114} (2015) no.13, 132002
doi:10.1103/PhysRevLett.114.132002
[arXiv:1411.3402 [hep-lat]].
%123 citations counted in INSPIRE as of 28 Sep 2020

%\cite{Miyahara:2015bya}
\bibitem{Miyahara:2015bya}
K.~Miyahara and T.~Hyodo,
%``Structure of \ensuremath{\Lambda}(1405) and construction of $\overline{K}N$ local potential based on chiral SU(3) dynamics,''
Phys. Rev. C \textbf{93} (2016) no.1, 015201
doi:10.1103/PhysRevC.93.015201
[arXiv:1506.05724 [nucl-th]].
%37 citations counted in INSPIRE as of 28 Sep 2020

%pLambda
%\cite{Munzer:2017hbl}
\bibitem{Munzer:2017hbl}
R.~M\"unzer, L.~Fabbietti, E.~Epple, S.~Lu, P.~Klose, F.~Hauenstein, N.~Herrmann, D.~Grzonka, Y.~Leifels and M.~Maggiora, \textit{et al.}
%``Determination of N* amplitudes from associated strangeness production in p+p collisions,''
Phys. Lett. B \textbf{785} (2018), 574-580
doi:10.1016/j.physletb.2018.08.068
[arXiv:1703.01978 [nucl-ex]].
%10 citations counted in INSPIRE as of 30 Sep 2020

%\cite{VanBuren:2005sk}
\bibitem{VanBuren:2005sk}
G.~Van Buren [STAR],
%``The Ratio Sigma0 / Lambda at RHIC,''
Rom. Rep. Phys. \textbf{58} (2006), 069-074
[arXiv:nucl-ex/0512018 [nucl-ex]].
%5 citations counted in INSPIRE as of 30 Sep 2020

%\cite{Borissov:2019dcv}
\bibitem{Borissov:2019dcv}
A.~Borissov [ALICE],
%``Production of $\Sigma^0$ Hyperons at LHC with ALICE,''
EPJ Web Conf. \textbf{222} (2019), 02002
doi:10.1051/epjconf/201922202002
%0 citations counted in INSPIRE as of 30 Sep 2020

%Neutron stars chapter

\bibitem{Ozel:2016oaf}
F.~Özel and P.~Freire, ``{Masses, Radii, and the Equation of State of Neutron
  Stars},'' \href{http://dx.doi.org/10.1146/annurev-astro-081915-023322}{{\em
  Ann. Rev. Astron. Astrophys.} {\bfseries 54} (2016) 401--440},
  \href{http://arxiv.org/abs/1603.02698}{{\ttfamily arXiv:1603.02698
  [astro-ph.HE]}}.

\bibitem{Riley:2019yda}
T.~E. Riley {\em et~al.}, ``{A $NICER$ View of PSR J0030+0451: Millisecond
  Pulsar Parameter Estimation},''
  \href{http://dx.doi.org/10.3847/2041-8213/ab481c}{{\em Astrophys. J. Lett.}
  {\bfseries 887} no.~1, (2019) L21},
  \href{http://arxiv.org/abs/1912.05702}{{\ttfamily arXiv:1912.05702
  [astro-ph.HE]}}.

\bibitem{Djapo:2008au}
H.~Djapo, B.-J. Schaefer, and J.~Wambach, ``{On the appearance of hyperons in
  neutron stars},'' \href{http://dx.doi.org/10.1103/PhysRevC.81.035803}{{\em
  Phys. Rev. C} {\bfseries 81} (2010) 035803},
  \href{http://arxiv.org/abs/0811.2939}{{\ttfamily arXiv:0811.2939 [nucl-th]}}.

\bibitem{Tolos:2020aln}
L.~Tolos and L.~Fabbietti, ``{Strangeness in Nuclei and Neutron Stars},''
  \href{http://dx.doi.org/10.1016/j.ppnp.2020.103770}{{\em Prog. Part. Nucl.
  Phys.} {\bfseries 112} (2020) 103770},
  \href{http://arxiv.org/abs/2002.09223}{{\ttfamily arXiv:2002.09223
  [nucl-ex]}}.

\bibitem{NS1Demorest:2010bx}
P.~Demorest, T.~Pennucci, S.~Ransom, M.~Roberts, and J.~Hessels, ``{Shapiro
  Delay Measurement of A Two Solar Mass Neutron Star},''
  \href{http://dx.doi.org/10.1038/nature09466}{{\em Nature} {\bfseries 467}
  (2010) 1081--1083}, \href{http://arxiv.org/abs/1010.5788}{{\ttfamily
  arXiv:1010.5788 [astro-ph.HE]}}.

\bibitem{NS2Antoniadis:2013pzd}
J.~Antoniadis {\em et~al.}, ``{A Massive Pulsar in a Compact Relativistic
  Binary},'' \href{http://dx.doi.org/10.1126/science.1233232}{{\em Science}
  {\bfseries 340} (2013) 6131},
  \href{http://arxiv.org/abs/1304.6875}{{\ttfamily arXiv:1304.6875
  [astro-ph.HE]}}.

\bibitem{NS3Cromartie:2019kug}
H.~T. Cromartie {\em et~al.}, ``{Relativistic Shapiro delay measurements of an
  extremely massive millisecond pulsar},''
  \href{http://dx.doi.org/10.1038/s41550-019-0880-2}{{\em Nature Astron.}
  {\bfseries 4} no.~1, (2019) 72--76},
  \href{http://arxiv.org/abs/1904.06759}{{\ttfamily arXiv:1904.06759
  [astro-ph.HE]}}.

\bibitem{Weissenborn:2011kb}
S.~Weissenborn, D.~Chatterjee, and J.~Schaffner-Bielich, ``{Hyperons and
  massive neutron stars: the role of hyperon potentials},''
  \href{http://dx.doi.org/10.1016/j.nuclphysa.2012.02.012}{{\em Nucl. Phys. A}
  {\bfseries 881} (2012) 62--77},
  \href{http://arxiv.org/abs/1111.6049}{{\ttfamily arXiv:1111.6049
  [astro-ph.HE]}}.

\bibitem{Weissenborn:2011ut}
S.~Weissenborn, D.~Chatterjee, and J.~Schaffner-Bielich, ``{Hyperons and
  massive neutron stars: vector repulsion and SU(3) symmetry},''
  \href{http://dx.doi.org/10.1103/PhysRevC.85.065802}{{\em Phys. Rev. C}
  {\bfseries 85} no.~6, (2012) 065802},
  \href{http://arxiv.org/abs/1112.0234}{{\ttfamily arXiv:1112.0234
  [astro-ph.HE]}}. [Erratum: Phys.Rev.C 90, 019904 (2014)].

%\cite{Haidenbauer:2016vfq}
\bibitem{Haidenbauer:2016vfq}
J.~Haidenbauer, U.~G.~Mei\ss{}ner, N.~Kaiser and W.~Weise,
%``Lambda-nuclear interactions and hyperon puzzle in neutron stars,''
Eur. Phys. J. A \textbf{53} (2017) no.6, 121
doi:10.1140/epja/i2017-12316-4
[arXiv:1612.03758 [nucl-th]].
%31 citations counted in INSPIRE as of 03 Oct 2020


%\cite{Lonardoni:2014bwa}
\bibitem{Lonardoni:2014bwa}
D.~Lonardoni, A.~Lovato, S.~Gandolfi and F.~Pederiva,
%``Hyperon Puzzle: Hints from Quantum Monte Carlo Calculations,''
Phys. Rev. Lett. \textbf{114} (2015) no.9, 092301
doi:10.1103/PhysRevLett.114.092301
[arXiv:1407.4448 [nucl-th]].
%165 citations counted in INSPIRE as of 03 Oct 2020

%\cite{Sasaki:2019qnh}
\bibitem{Sasaki:2019qnh}
K.~Sasaki \textit{et al.} [HAL QCD],
%``$\Lambda\Lambda$ and N$\Xi$ interactions from Lattice QCD near the physical point,''
Nucl. Phys. A \textbf{998} (2020), 121737
doi:10.1016/j.nuclphysa.2020.121737
[arXiv:1912.08630 [hep-lat]].
%17 citations counted in INSPIRE as of 03 Oct 2020

%\cite{Inoue:2016qxt}
\bibitem{Inoue:2016qxt}
T.~Inoue [LATTICE-HALQCD],
%``Hyperon single-particle potentials from QCD on lattice,''
PoS \textbf{INPC2016} (2016), 277
doi:10.22323/1.281.0277
[arXiv:1612.08399 [hep-lat]].
%10 citations counted in INSPIRE as of 04 Oct 2020

\end{thebibliography}

